Style Example-Guided Text Generation using Generative Adversarial Transformers

We introduce a language generative model framework for generating a styled paragraph based on a context sentence and a style reference example. The framework consists of a style encoder and a texts decoder. The style encoder extracts a style code from the reference example, and the text decoder generates texts based on the style code and the context. We propose a novel objective function to train our framework. We also investigate different network design choices. We conduct extensive experimental validation with comparison to strong baselines to validate the effectiveness of the proposed framework using a newly collected dataset with diverse text styles. Both code and dataset will be released upon publication.

==> figtex/fig_AdaLN.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=.7\linewidth]{figures/AdaIN.pdf}
    %\vspace{-0.5cm}
    \caption{AdaIN.}
    %\vspace{-0.3cm}
    \label{fig:AdaLN}
\end{figure}

==> figtex/fig_amt_style.tex <==
\begin{table}[!t]
    \setlength\extrarowheight{1pt}
    \setlength{\tabcolsep}{2pt}
	\centering
	\begin{tabular}{c || c | c | c |}
\hline
	    \multicolumn{1}{|c||}{(\%)}& Model D & SC & Random\\ 
	    \hline
	    \multicolumn{1}{|c||}{$3$-style by reference}&  56 & 52 & 50 \\ \hline
	    \multicolumn{1}{|c||}{$3$-style by category}&  65 & 54 & 50 \\ \hline	    
	    \multicolumn{1}{|c||}{$21$-style by reference}& 66 & 49 & 50 \\ \hline
	    \multicolumn{1}{|c||}{$21$-style by category}& 69 & 50 & 50 \\ \hline
	\end{tabular}
	\caption{Human Study on Styles classification. Random denotes the accuracy for random guess.}
	\label{tab:amt_style}
\end{table}

==> figtex/fig_example_output.tex <==
\begin{tabular}{cc}
\missingfigure[figwidth=2in]{3 example output}& \missingfigure[figwidth=2in]{21 example output}
\end{tabular}

==> figtex/fig_output_novelty.tex <==
\begin{table}[h]
    \setlength\extrarowheight{1pt}
    \setlength{\tabcolsep}{2pt}
	\centering
	\begin{tabular}{c || c | c | c | c | c | c | c | c | c |}
	    \cline{2-10}
	    & Model A  & Model B & Model C & Model D & G-GPT-2  & S-GPT-2 & SC & UB & LB\\ 
	    \hline
	    \multicolumn{1}{|c||}{\texttt{3-Style}}& 27.92 & 30.48 & 31.19 & 28.00 & 31.41 & 31.24 & 31.20 & 33.45 & 17.07 \\ \hline	    
	    \multicolumn{1}{|c||}{\texttt{21-Style}}& 28.10 & 29.80 & 29.81 & 27.53 & 31.46 & -- & 30.92 & 31.46 & 15.13 \\ \hline
	\end{tabular}
	\caption{Content Novelty. UB denotes upper bound computed by pretrained GPT-2 embedding on cross style paragraphs. LB denotes lower bound computed by pretrained GPT-2 embedding on cross paragraph in the same document.}
	\label{tab:novelty}
\end{table}
